Contractions, Removals and How to Certify 3-Connectivity in Linear Time

It is well-known as an existence result that every 3-connected graph G=(V,E) on more than 4 vertices admits a sequence of contractions and a sequence of removal operations to K_4 such that every intermediate graph is 3-connected. We show that both sequences can be computed in optimal time, improving the previously best known running times of O(|V|^2) to O(|V|+|E|). This settles also the open question of finding a linear time 3-connectivity test that is certifying and extends to a certifying 3-edge-connectivity test in the same time. The certificates used are easy to verify in time O(|E|).

==> Certifying.tex <==
We use construction sequences in the path representation as a certificate for the $3$-connectedness of graphs. This leads to a new, certifying method for testing graphs on being $3$-connected. The total running time of this method is $O(n^2)$, however this is dominated by the time needed for finding the construction sequence and every improvement made there will automatically result in a faster $3$-connectedness test. The input graph is a multigraph and does not have to be biconnected nor connected. We follow the steps:

\begin{itemize}
	\item Apply preprocessing of Nagamochi and Ibaraki and get $G$ in $O(n+m)$\\(this is only used to improve the running time)
	\item Try to compute a $K_4$-subdivision $S_0$ in $G$ and prescribe it in $O(n)$
	\begin{itemize}
		\item Failure: Return a separation pair
	\end{itemize}
	\item Try to compute a construction sequence from $S_0$ to $G$ in $O(n^2)$
	\begin{itemize}
		\item Success: Return the construction sequence
		\item Failure: Return a separation pair
	\end{itemize}
\end{itemize}

\begin{wrapfigure}[16]{R}{3cm}
	\vspace{-1cm}
	\centering
	\includegraphics[scale=0.6]{./Pictures/FindK4}
	\caption{Finding a $K_4$-subdivision. Dashed edges can be (empty) paths, arcs depict backedges.}
	\label{fig:findk4}
\end{wrapfigure}

The preprocessing step preserves the graph to be $3$-connected or to be not $3$-connected. We first describe how to find a $K_4$-subdivision by one Depth First Search (DFS), which as a byproduct eliminates self-loops and parallel edges and sorts out graphs that are not connected or have vertices with degree at most $2$. Let $a$ (resp. $b$) be the vertex in the DFS-tree $T$ that is visited first (resp. second). If $G$ is $3$-connected, then $a$ and $b$ have exactly one child, otherwise they form a separation pair. We choose two arbitrary neighbors $c$ and $d$ of $a$ that are different from $b$ (see Figure~\ref{fig:findk4}). W.l.o.g., let $d$ be visited later by the DFS than $c$. Let $i \neq b$ the least common ancestor of $c$ and $d$ in $T$. As $d \neq i$ must hold, let $j$ be the child of $i$ that is contained in the path $i \rightarrow d$ in $T$.

If $G$ is $3$-connected, we can find a backedge $e$ that starts on a vertex $z$ in the subtree rooted at $j$ and ends on an inner vertex $z'$ of $a \rightarrow i$ in time $O(n)$. If $e$ does not exist, $a$ and $i$ form a separation pair, otherwise we have found a $K_4$-subdivision with real vertices $a$, $i$, $z$ and $z'$. The paths connecting this real vertices in $T$ together with the three visited backedges constitute the $6$ paths of the $K_4$-subdivision.

Once the $K_4$-subdivision $S_0$ is found, we follow the lines of Theorem~\ref{multipleconstruction} and try to construct the path representation $C_0,\ldots,C_{z-1}$. If favored, this can be transformed to an edge representation in $O(m)$ later. We assign an index for every link and store it on each of the inner vertices of that link. Moreover, we maintain pointers for each link to its end vertices.

In case $H \neq \emph{smooth}(H)$ of Theorem~\ref{multipleconstruction} we pick an arbitrary vertex $x$ of degree two. Let $T = a \rightarrow b$ be the link that contains $x$ and let $W$ be the set of vertices $V(H) \setminus V(T)$ minus all vertices in parallel links of $T$ (see Figure~\ref{fig:dfs}). We compute the path $P = x \rightarrow y'$ by temporarily deleting $a$ and $b$ and performing a DFS on $x$ that stops on the first vertex $y' \in W$. We can check whether a vertex lies in a parallel link of $T$ in constant time by comparing the end vertices of its containing link with $a$ and $b$. Thus, the subpath $x' \rightarrow y'$ with $x'$ being the last vertex contained in $T$ or in a parallel link of $T$ is a \BG-path and can be found efficiently. The links and their indices can be updated in $O(n)$.

Similarly, in case $H = \emph{smooth}(H)$ we delete temporarily all edges in $E(H)$ and start a DFS on a vertex $x \in V(H)$ that has an incident edge in the remaining graph. The traversal is stopped on the first vertex $y \in V(H) \setminus \{x\}$. The path $x \rightarrow y$ is then the desired \BG-path and we conclude that for $3$-connected graphs the construction sequence can be found in time $O(n^2)$.

Otherwise, $G$ is not $3$-connected and no construction sequence can exist with Theorem~\ref{constructions}. In that case a DFS starting at vertex $x$ fails to find a new \BG-path for some subdivision $H \subset G$. If $H \neq \emph{smooth}(H)$, the end vertices of the link that contains $x$ must form a separation pair. Otherwise, $H = \emph{smooth}(H)$ and $x$ must be a cut vertex. Thus, if $G$ is not $3$-connected, the algorithm returns always a separation pair or cut vertex.

We show how to construct the basic construction sequence~\eqref{theoremitem2} when $G$ is simple.

\begin{lemma}\label{transform}
For simple graphs $G$, the construction sequences~\eqref{theoremitem1} and~\eqref{theoremitem2} can be transformed into each other in $O(m)$.
\end{lemma}
\begin{proof}
Let the construction sequence~\eqref{theoremitem1} in the path representation be given. For each \BG-path $P$, its position in the construction sequence and a pointer to the first \BG-path $F(P)$ that ends at an inner vertex of $P$ (if that path exists) is stored. We define the position of each link of $S_0$ as $0$. Performing a bucket sort on the end vertices of \BG-paths with lower id followed by a stable bucket sort on the remaining end vertices gives a list of paths sorted in lexicographic order of the end vertex ids. This list can be used to efficiently group paths that have the same end vertices.

Let $S_{ab}$ be the set of all \BG-paths and links of $S_0$ having end vertices $a$ and $b$. We apply the following procedure: If a path $P \in S_{ab}$ has length one and does not have the first position of all paths in $S_{ab}$, we append it to the end of the construction sequence and remove it from $S_{ab}$. This does not harm the construction sequence, since $a$ and $b$ were already real and $P$ has no inner vertices.

The path with the first position in $S_{ab}$ cannot lead to a non-basic operation. We look at all other paths $P \in S_{ab}$, which are possibly non-basic, but must contain an inner vertex $w$ that is end vertex of the subsequent \BG-path $F(P) = v~\rightarrow~w$. Without harming the construction sequence, $P$ can be moved to the position of $F(P)$, since $a$ and $b$ were already real and no inner vertex of $P$ is part of a \BG-path before $F(P)$ is applied. If $v$ is real at the point in time when $F(P)$ is applied, we can glue $P$ and $F(P)$ together to an expand operation, which is basic due to its new vertex $w$. Otherwise, $v$ is an inner vertex of a link (see Figure~\ref{fig:notexpand}) and $P$ and $F(P)$ can be replaced with the two \BG-paths $v \rightarrow a$ and $bw$. Both \BG-paths are basic, since they contain end vertices of degree $2$.

Conversely, the three internally vertex-disjoint paths of each expand operation can be easily split into two \BG-paths, possibly inducing non-basic operations.
\qed\end{proof}

\begin{wrapfigure}[10]{R}{3cm}
	\vspace{-0.7cm}
	\centering
	\includegraphics[scale=0.6]{./Pictures/NoExpand}
	\caption{No expand operation can be formed.}
	\label{fig:notexpand}
\end{wrapfigure}

\begin{theorem}\label{algorithm}
The construction sequences~\eqref{theoremitem1} and~\eqref{theoremitem2} can be computed in $O(n^2)$ and establish a certifying $3$-connectedness test with the same running time.
\end{theorem}


\subsection{Verifying the Construction Sequence}
It is essential for a certificate that it can be easily validated. We could do this by transforming the path representation to the edge representation using Lemma~\ref{representation} and checking the \BG-operations on being valid by comparing indices, but there is a more direct way. First, it can be checked in linear time that all \BG-paths $C_0,\ldots,C_{z-1}$ are paths in $G$ and that these paths partition $E(G) \setminus E(S_0)$. We try to remove the \BG-paths $C_{z-1},\ldots,C_0$ from $G$ in that order (i.\,e., we delete the paths followed by smoothing its end vertices). If the certificate is valid, this is well defined as all removed \BG-paths are then edges. On the other hand we can detect longer \BG-paths $|C_i| \geq 2$ before their removal, in which case the certificate is not valid, since then the inner vertices of $C_i$ are not attached to \BG-paths $C_j$, $j > i$.

\begin{wrapfigure}[15]{R}{3.5cm}
	\centering
	\subfigure[Either $a$ or $b$ has degree $2$.]{
		\includegraphics[scale=0.6]{./Pictures/Verifying1}
		\label{fig:check1}
	}
	\hfill
		\subfigure[Both $a$ and $b$ have degree $2$.]{
		\includegraphics[scale=0.6]{./Pictures/Verifying2}
		\label{fig:check2}
	}
	\caption{Cases where~\ref{bgpathdefinition}.\ref{bgpathdefinition2} fails when $a \in N(b)$.}
	\label{fig:check}
\end{wrapfigure}

We verify that every removed $C_i = ab$ corresponds to a \BG-operation by using Definition~\ref{bgpathdefinition} of \BG-paths, and start with checking that $a$ and $b$ lie in our current subgraph for condition~\ref{bgpathdefinition}.\ref{bgpathdefinition1}.

Conditions~\ref{bgpathdefinition}.\ref{bgpathdefinition2} and~\ref{bgpathdefinition}.\ref{bgpathdefinition3} can now be checked in constant time: Consider the situation immediately after the deletion of $ab$, but before smoothing $a$ and $b$. Then all links in our subgraph are single edges, except possibly the ones containing $a$ and $b$ as inner vertices.

Therefore,~\ref{bgpathdefinition}.\ref{bgpathdefinition2} is not met for $C_i$ if $a$ is a neighbor of $b$ and at least one of the vertices $a$ and $b$ has degree two (see Figures~\ref{fig:check} for possible configurations). Condition~\ref{bgpathdefinition}.\ref{bgpathdefinition3} is not met if $N(a) = N(b)$ and both $a$ and $b$ have degree two. Both conditions can be easily checked in constant time. Note that encountering proper \BG-paths $C_{z-1},\ldots,C_i$ does not necessarily imply that the current subgraph is $3$-connected, since false \BG-paths $C_j$, $j < i$, can exist.

It remains to validate that the graph after removing all \BG-paths is the $K_4$. This can done in constant time by checking it on being simple and having exactly $4$ vertices of degree three.

\begin{theorem}\label{verifying}
The construction sequences~\eqref{removals}-\eqref{theoremitem2} can be checked on validity in time linearly dependent on their length.
\end{theorem}
